A HeARTfelt Robot: Social Robot-Driven Deep Emotional Art Reflection with Children

Social-emotional learning (SEL) skills are essential for children to develop to provide a foundation for future relational and academic success. Using art as a medium for creation or as a topic to provoke conversation is a well-known method of SEL learning. Similarly, social robots have been used to teach SEL competencies like empathy, but the combination of art and social robotics has been minimally explored. In this paper, we present a novel child-robot interaction designed to foster empathy and promote SEL competencies via a conversation about art scaffolded by a social robot. Participants (N=11, age range: 7-11) conversed with a social robot about emotional and neutral art. Analysis of video and speech data demonstrated that this interaction design successfully engaged children in the practice of SEL skills, like emotion recognition and self-awareness, and greater rates of empathetic reasoning were observed when children engaged with the robot about emotional art. This study demonstrated that art-based reflection with a social robot, particularly on emotional art, can foster empathy in children, and interactions with a social robot help alleviate discomfort when sharing deep or vulnerable emotions.

==> tables/themes.tex <==
\begin{table}[]
\begin{tabular}{lllll}
\textbf{Theme} & \textbf{Definition} &  &  &  \\
Study participation & Participant mentions the current, previous, or future studies conducted at MIT &  &  &  \\
Quality time & Participant mentions spending time with their family, friends, pets, etc &  &  &  \\
Life Experience & Participant mentions a passing incident they've had at least once in their life (e.g. went to supermarket, broke a bone, etc.) &  &  &  \\
Creating & Participant mentions creating something themselves (e.g. baking, drawing, filming videos, etc.) &  &  &  \\
Viewing art & Participant mentions viewing a piece of artwork &  &  &  \\
Hobbies & Participant mentions their hobbies &  &  &  \\
School & Participant mentions an incident that occured or is related to their school &  &  &  \\
Other (N/A) & Doesn't fall into any category &  &  &  \\
 &  &  &  &  \\
 &  &  &  &  \\
 &  &  &  &  \\
 &  &  &  & 
\end{tabular}
\caption{}
\label{tab:themes}
\end{table}
